Global and Local Structure Learning for Sparse Tensor Completion

How can we accurately complete tensors by learning relationships of dimensions along each mode? Tensor completion, a widely studied problem, is to predict missing entries in incomplete tensors. Tensor decomposition methods, fundamental tensor analysis tools, have been actively developed to solve tensor completion tasks. However, standard tensor decomposition models have not been designed to learn relationships of dimensions along each mode, which limits to accurate tensor completion. Also, previously developed tensor decomposition models have required prior knowledge between relations within dimensions to model the relations, expensive to obtain. This paper proposes TGL (Tensor Decomposition Learning Global and Local Structures) to accurately predict missing entries in tensors. TGL reconstructs a tensor with factor matrices which learn local structures with GNN without prior knowledges. Extensive experiments are conducted to evaluate TGL with baselines and datasets.

==> 050related.tex <==


I will briefly describe literature of tensor completion based on tensor decomposition methods and
review Graph Convolutional Networks (GCNs).

\subsection{Tensor Completion}
%Tensor completion is one of the main problems in numerous tensor related applications~\cite{song2019tensor}./
Various tensor decomposition methods have been developed to solve tensor completion problems in numerous tensor related applications~\cite{song2019tensor, zhou2017tensor}
ranging from Recommender Systems~\cite{liu2019costco}, Computer Vision~\cite{vasilescu2002multilinear}, and Air Quality Analysis~\cite{ahn2022time}.
Even though, various tensor completion methods based on tensor decomposition methods have been developed, 
1) those learn relation of dimensions of specific mode, and 
2) those are applicable when only prior knowledges have been known
while the proposed method learn relations between dimensions of any mode without prior knowledges and assumptions.


\subsection{Graph Convolutional Networks}
GCNs~\cite{scarselli2008graph, defferrard2016convolutional} are a type of neural networks to deal with graph-structured data.
The layers of GCN are called convolutional layers which generalize operations of Convolutional Neural Networks (CNN)
because they both effectively learn features of neighborhoods.
The main difference between those is that CNNs are operated on Euclidean or grid-like structure data while
GCNs work on Non-euclidean structure data since nodes of graphs are not ordered and are irregular structure 
(e.g., each node has different numbers of neighbors).
%
Beside GCNs models, various types of graph neural networks have been developed in recent years such as
graph attention model and graph recurrent neural networks, graph generative models.
%
The reason why I used GCN for learning relations of dimensions is that each dimension of tensor is irregular such that
I do not know which dimension is related to which dimensions and how many dimensions are related together and GCNs are effectively learn this irregular structures.

